Relax-and-split method for nonsmooth nonconvex problems

We develop and analyze a new `relax-and-split' (RS) approach for compositions of separable nonconvex nonsmooth functions with linear maps. RS uses a relaxation technique together with partial minimization, and brings classic techniques including direct factorization, matrix decompositions, and fast iterative methods to bear on nonsmooth nonconvex problems. We also extend the approach to trimmed nonconvex-composite formulations; the resulting Trimmed RS (TRS) can fit models while detecting outliers in the data. We then test RS and TRS on a diverse set of applications: (1) phase retrieval, (2) stochastic shortest path problems, (3) semi-supervised classification, and (4) new clustering approaches. RS/TRS can be applied to models with very weak functional assumptions, are easy to implement, competitive with existing methods, and enable a new level of modeling formulations to be put forward to address emerging challenges in the mathematical sciences.

==> extra.tex <==
\subsection{Exact RPCA}
\label{sec:rpca}
Principal component analysis (PCA) is a fundamental data decomposition technique implemented via the SVD.  
However, in the presence of sparse `outliers', robust PCA (RPCA) is applied
to  deconvolve the data into a low rank and sparse component. 
RPCA has applications to alignment of occluded images \citep{peng2012rasl},
scene triangulation \citep{zhang2012tilt}, model selection \citep{chandrasekaran2009sparse}, face recognition \citep{turk1991face} and document indexing \citep{candes2011robust}.
In computer vision, it is widely used in background/foreground separation \citep{bouwmans2017decomposition}
to separate moving objects from their surroundings.

%Algorithm developed for RPCA usually is gradient based and do not enjoy the efficiency of the SVD.
There are a wide variety of RPCA formulations algorithms (see e.g.~\cite{bouwmans2016handbook}), 
including  primal-dual methods, gradient-based methods,  and level-set optimization.  Algorithm~\ref{alg:pg_w} is unique among these
because it solves the x-subproblem using the SVD (and its randomized variants). 
It brings the classic direct decomposition back to solve nonsmooth, nonconvex matrix factorization problems. 

Denote $D\in\R^{m \times n}$ as the video stream, where each of $m$ frames is reshaped to be a vector of size $n$.
Consider the exact RPCA formulation,
\begin{equation}
\label{eq:exact_rpca}
\min_{L,R} \|D - LR\|_1
\end{equation}
where $L\in\R^{m\times k}$ and $R\in\R^{k\times n}$. $\ell_1$ norm gives an exact fit for many datapoints, forcing them to be background; at the same time allows occasional large residuals, which reveals the sparse foreground. 
We consider the relaxed formulation
\begin{equation}
\label{eq:exact_rpca_relax}
\min_{L,R,W} \|D - W\|_1 + \frac{1}{2\nu}\|W - LR\|_F^2.
\end{equation}
Algorithm~\ref{alg:pg_w} for \eqref{eq:exact_rpca_relax} requires solving a least squares matrix factorization problem in $(L,R)$;  the SVD gives a closed form solution: 
\[
W = U\Sigma V\T, \quad L = U\Sigma^{1/2}, \quad R = \Sigma^{1/2}V\T.
\]

In this experiment, we pick 202 images from the data set\footnote{Publicly available at \url{http://vis-www.cs.umass.edu/~narayana/castanza/I2Rdataset/} \label{IR_dataset}}, $D\in\R^{20480\times 202}$. The results are shown in Figure~\ref{fig:rpca_con_his} and Figure~\ref{fig:rpca_result}.

\begin{figure}[h]
\centering
\includegraphics[width=0.47\textwidth]{figs/rpca_obj_his.pdf}
\includegraphics[width=0.47\textwidth]{figs/rpca_err_his.pdf}
\caption{\label{fig:rpca_con_his} Convergence history of Algorithm~\ref{alg:pg_w} applied to \eqref{eq:exact_rpca_relax}.
Objective value (left) and optimality condition (right) are plotted as a function of iterations.}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figs/back.jpg}
\includegraphics[width=0.4\textwidth]{figs/binary.jpg}
\caption{\label{fig:rpca_result} Result for background/foreground separation. Background (left) and foreground (right) are plotted. For foreground, binary thresholding is used to highlight the quality of the separation; every pixel has value $0$ or $1$.}
\end{figure}

In Figure~\ref{fig:rpca_con_his}, we see a fast linear convergence rate, and Algorithm~\ref{alg:pg_w} solves the problem within 15 iterations. We obtain the background from $LR$ and the foreground from $W-LR$. The separation is shown in Figure~\ref{fig:rpca_result}; the van is plotted using binary thresholding, to emphasize that the quality of the separation. 

\section{Conclusion} This paper develops an efficient methodology for solving nonsmooth, nonconvex problems in a wide range of settings. Using a smoothing relaxation, we partially minimize in the primary variables of interest, which seems expensive by pays off both in theoretical rates and practical performance. The original problem is decoupled into least squares optimization and proximal operators;  the former can be solved using direct factorization, iterative methods, or matrix decompositions (e.g. rSVD), while the latter are separable and straightforward to implement in all motivating examples. The approach works particularly well for problems with sharp features, including S$^3$VM, phase retrieval, stochastic shortest path problems, and exact RPCA. 

We derived theoretical results for the \underline{nonconvex composite} class, under a range of assumptions, but many practical and theoretical questions are left open to future work. In particular, (1) nonsmooth regularization must be better addressed; (2) certain classes of problems such as the RPCA are not covered under the theory but work very well in practice and (3) the role of approximation and continuation must be further analyzed. The current manuscript is best viewed as a starting point to develop a new generation of fast algorithms for nonsmooth, nonconvex problems. 

\bigskip


==> min_section.tex <==
\section{The Second Composite Class}

In this section, we consider a consider the model:
\begin{align}\label{eq:concavecomp}
%F(x) = \inf_{\xi} (h(c(x; \xi), \xi)),
F(x) =  g(h_{1}(c_{1}(x)), \ldots, h_{n}(c_{n}(x))),
\end{align}
where  
\begin{enumerate}
%\item $I_i \subseteq \NN$ is a collection of indices.
\item $g : \RR_+^{n} \rightarrow \RR$ is a continuous concave functions such $\dom\left(g^\ast\right) \subseteq \RR_-^{n} $ and $B := \sup_{x \in \dom\left(g^\ast\right)}\|x\| < \infty.$
\item $h_i : R^{n_{i}} \rightarrow \RR$ are $L$-Lipchitz and convex.
\item $c_{i}\colon\R^{d}\to\R^{n_{i}}$ are $C^1$-smooth with the Jacobian map $\nabla c_{i}$ that is $\beta$-Lipschitz continuous.
\end{enumerate}

We describe a few examples of this class.
\begin{example}[Real Phase Retrieval] Consider the real analogue of complex phase retrieval problem presented in Example~\ref{ex:phase_retrieval}, which takes the form
$$
F(x) = \sum_{i=1}^n |b_i - |\dotp{a_i, x}||.
$$
This loss is an instance of Problem~\eqref{eq:concavecomp} with $n = 2d$, $c_i := I$, and 
\begin{align*}
g(y_1, y_2, \ldots, y_{2d-1}, y_{2d}) = \frac{1}{n}\sum_{i=1}^d \min\{y_{2i-1}, y_{2i}\}, &&  h_{2i-1} := |\dotp{a_i, x}+b_i|, && h_{2i} := |\dotp{a_{i}, x}-b_i|.
\end{align*}
This particular splitting follows after noticing that the primitive satisfies $|b_i - |\dotp{a_i, x}|| = \min\{ |b_i - |\dotp{a_i, x}||, |b_i + |\dotp{a_i, x}||\}.$
\end{example}

\begin{example}[Trimmed Model Fitting]
Let $t \in [n]$ and consider the following trimmed model fitting problem~\cite{????}, which seeks to detect and remove contaminated data from a training set while simultaneously fitting a trimmed model on the uncontaminated data that remains:
\begin{align*}
\minimize_{x} &\; F(x) := \frac{1}{t}\sum_{i=1}^t h_{i:n}(c_{i:n}(x)))\\
\text{subject to:} &\; h_{1:n}(c_{1:n}(x)) \leq \ldots \leq  h_{n:n}(c_{n:n}(x)).
\end{align*}
In this case, the concave outer function $g :\RR^n \rightarrow \RR$ is simply the function that sums the smallest $t$ elements of a vector of length $n$.
\end{example}

\begin{example}[Nonlinear Complementarity]
Consider the nonlinear complementarity problem
\begin{align*}
0 \leq F(x) \perp G(x) \geq 0 
\end{align*}
i.e., we want to find $x$ such that $F(x), G(x) \geq 0$ and $\dotp{F(x), G(x)} = 0$. This problem cones from the inclusion 
\begin{align*}
0 \in  N_{\RR_{\geq 0}}(G(x)) + F(x) .
\end{align*}
This problem can be reformulated as the componentwise min
\begin{align*}
\min(F(x), G(x)) = 0.
\end{align*}
This can be reformulated equivalently as, 
\begin{align*}
\minimize_x\left\{\sum_{i=1}^n\min(F_i(x), G_i(x)) + 2\max(-F_i(x), 0) + 2\max(-G_i(x), 0)\right\}.
\end{align*}
%So let $f(x) = \max(x, 0)$. We know how to compute the function $h_{-f}(v, r)$. Therefore, the above problem can be reformulated as 
%\begin{align*}
%\minimize_{\substack{x, w^1 \geq 0, w^2 \geq 0,\\ w^1_i + w_2^i = 1, v^1, v^2\\
%r^1, r^2}}&\sum_{i=1}^n \biggl\{w_i^1F_i(x) + w_i^2 G_i(x) + 2\left(h_{-f}(v_i^1, r_i^1) + h_{-f}(v_i^2, r_i^2)\right) \\
%&\hspace{20pt}+ v_i^1F_i(x)+ \frac{r_i^1}{2}F_i(x)^2+ v_i^2G_i(x) + \frac{r_i^2}{2}G_i(x)^2 \biggr\}
%\end{align*}
\end{example}


Consider the surrogate function
\begin{align*}
F(x, w)  := \sum_{i=1}^n w_{i}h_{i}(c_{i}(x)) + (-g)^\ast(-w).
\end{align*}
The connection between $F(x)$ and $F(x, w)$ becomes apparent through the relationship 
\begin{align*}
\inf_x F(x) = \inf_x g(h_{1}(c_{1}(x)), \ldots, h_{n}(c_{n}(x))) &= \inf_{x, v}\left\{ -\dotp{v, (h_{1}(c_{1}(x)), \ldots, h_{n}(c_{n}(x)))} + (-g)^\ast(v)\right\}\\
&=\inf_{x, w}\left\{ \sum_{i=1}w_ih_{i}(c_{i}(x)) + (-g)^\ast(-w)\right\} := \inf_{x, w} F(x, w).
\end{align*}
Clearly, any minimizing pair $(x^\ast, w^\ast)$ of the latter problem leads to a minimizer $x^\ast$ of the former. 

As in Algorithm~\ref{alg:COMP-PAM2}, the following linearization $F_{y}$ plays a key algorithmic role:
\begin{align*}
F_y(x, w)  :=\sum_{i=1}^n w_{i}h_{i}(c_{i}(y) + \nabla c_i(y)(x -y)) + (-g)^\ast(-w)
\end{align*}
As before, these linearizations enjoy the well-known approximation property; for a proof, see for example~\cite[Lemma 3.2]{comp_DP} or \cite[Lemma 1]{nest_GN}.
\begin{lemma}\label{lem:est_approx}
For any points $x$, $y$, $w$, the estimate holds:
$$
|F_y(x, w) - F(x,w) | \leq \frac{L\beta B}{2} \|y - x\|^2.
$$
\end{lemma}

We exploit this splitting in the following algorithm:
\begin{algorithm}[H]
  \caption{MinPAM:  Composite Proximal Alternating Minimization
    \label{alg:MIN_PAM}}
  \begin{algorithmic}[1]
    \Require{$x_0 \in \RR^{d},  \gamma>0 $.}
   % \Statex
  
   \Statex{Set $w^0 \in \am_{w} \; F(x^{0},w)$.}
    \Statex{{\bf Step $k$:} $(k\geq 0)$}
        \Statex \label{alg:main:line_PG} $\qquad$ Choose $w^{k+1} \in \am_{w} \; F(x^{k},w)$
 \Statex\label{alg:main:line_PL} $\qquad$ Set $x^{k+1} = \am_{x} \; F_{x_k}(x,w^{k+1})+ \frac{1}{2\gamma} \|x - x^k\|^2$
  \end{algorithmic}
\end{algorithm}


The following is a straightforward exercise.
\begin{lemma}[Weak Convexity]
For all $(\bar x, \bar w) \in \dom(F)$, we have
$$
\hat \partial F(\bar x, \bar w) =\hat  \partial_x F(\bar x, \bar w) \times\hat  \partial_w F(\bar x, \bar w).
$$
\end{lemma}
%\begin{proof}
%Let $v = (v_{\bar x}, v_{\bar w}) \in \partial F(\bar x, \bar w)$. Then clearly $v \in \hat  \partial_x F(\bar x,\bar  w) \times\hat  \partial_w F(\bar x, \bar w).$.
%
%Conversely, suppose that $v_{\bar x }\in \hat  \partial_x F(\bar x,\bar  w)$ and $v_{\bar w} \in \hat \partial_w F(\bar x, \bar w)$. Then 
%\begin{align*}
%F(x, w) &= w^T (h_i(c_i(x)))_i  + (-g)^\ast(-w) \\
%&= \bar w^T (h_i(c_i(x)))_i + (w -\bar  w)^T(h_i(c_i(x)))_i  + (-g)^\ast(-w) \\
%\end{align*}
%\end{proof}


Our now state and prove our convergence theorem. 
\begin{theorem}\label{thm:main_thm2}
The iterates $(x_k,w_k)$ generated by Algorithm~\ref{alg:COMP-PAM2} satisfy
\begin{equation}\label{eqn:summ2}
\sum_{k=0}^{\infty} \left(\frac{1}{\gamma_k} - \frac{L\beta B}{2}\right)\|x^{k+1}-x^k\|^2\leq F(x^0)-F^*,
\end{equation}
where we set $\displaystyle F^*:=\lf_{k\to\infty} F(x^k,w^k)$. Moreover, the following approximate stationarity condition holds: there exists $\hat x^{k+1}$ such that 
\begin{equation}\label{eqn:approx_stat2}
\left\{\begin{aligned}
\dist(0, \hat \partial_x F(\hat x^{k+1}, w^{k+1}))  &\leq  \left(3L\beta B  + \frac{1}{\gamma}\right)\| x^{k+1} - x^k\|  \\
 \|\hat x^{k+1} - x^{k+1} \|&\leq \| x^{k+1} - x^k\|\\
 \dist(0, \hat \partial_w F(\hat x^{k+1}, w^{k+1})) &\leq \|( h_{i}(c_{ij}(\hat x^{k+1})) - h_{i}(c_{i}(x^k))_{i}\|\\
  \|\hat x^{k+1} - x^{k} \|&\leq 2\| x^{k+1} - x^k\|\\
\end{aligned}\right\}.
\end{equation}
\end{theorem}
\begin{proof}
The proof follows the same outline as that of Theorem~\ref{thm:main_thm}; therefore omit some details.
For any index $k$, strong convexity of $F_{x^k}(\cdot,w^{k+1})+\frac{1}{2\gamma_k}\|\cdot-x^k\|^2$
implies
$$\left(F_{x^{k}}(x^{k+1},w^{k+1})+\frac{1}{2\gamma_k}\|x^{k+1}-x^k\|^2\right)+ \frac{1}{2\gamma}\|x^{k+1}-x^k\|^2\leq F_{x_k}(x^{k},w^{k+1})=F(x^k,w^{k+1})\leq F(x^k,w^{k}).$$
Combining this inequality with Lemma~\ref{lem:est_approx} yields 
\begin{align*}
F(x^{k+1}, w^{k+1})  \leq F_{x^k}(x^{k+1},w^{k+1}) + \frac{L\beta B }{2}\|x^{k+1} - x^k\|^2
%&\leq F_{x^k}(x^{k},w^{k+1})-\left(\frac{1}{2\gamma_k} - \frac{L\beta B \bar L}{2}\right) \|x^{k+1}-x^k\|^2\\
\leq F(x^{k},w^{k})-\left(\frac{1}{\gamma_k} - \frac{L\beta B}{2}\right)\|x^{k+1}-x^k\|^2.
\end{align*}
Rearranging as in the proof of Theorem~\ref{thm:main_thm} establishes \eqref{eqn:summ2}. 

%Observe that
%$$
%\frac{1}{\gamma}(x^{k} - x^{k+1}) \in \partial_{x} F(x^{k+1}, w^{k+1})
%$$
%Moreover, 
%%$$
%% \partial_w F(x^{k+1}, w^{k+1}) = h(c(x_{k+1}))  + N_{\Delta}(w^{k+1}) = h(c(x_{k}))  + N_{\Delta}(w^{k+1}) + h(c(x^{k}})) - h(c(x_{k}))
%%$$

We now establish the claimed stationary bounds. To do this, we apply the smooth variational principle to the function $\varphi(y) = F(y, w^{k+1}) + (1/2)\left(1/\gamma+ L\beta B \right)\| y - x^k\|^2$. In support of this goal, we notice that 
$$
\varphi(y) \geq F_{x_k}(y, w^{k+1})+ \frac{1}{2\gamma}\| y - x^k\|^2 \geq F_{x_k}(x^{k+1}, w^{k+1}) + \frac{1}{2\gamma}\| x^{k+1} - x^k\|^2.
$$
Hence, 
$$
\varphi(x^{k+1}) - \inf \varphi \leq  F(x^{k+1} , w^{k+1}) - F_{x_k}(x^{k+1}, w^{k+1}) +\frac{L\beta B}{2}\| x^{k+1} - x^k\|^2 \leq L\beta B\| x^{k+1} - x^k\|^2.
$$
Thus, by Lemma~\ref{lem:smooth_var_princ_damek} with $\varepsilon := L\beta B\| x^{k+1} - x^k\|^2$ and $\lambda = \| x^{k+1} - x^k\|$, the point 
$$
\hat x^{k+1} = \prox_{\frac{\lambda}{2\varepsilon} \varphi}(x^{k+1}),
$$
satisfies $\|\hat x^{k+1} - x^{k+1}\| \leq \lambda = \| x^{k+1} - x^k\|$ and 
\begin{align*}
&\dist(0, \partial \varphi(\hat x^{k+1})) \leq \frac{2\varepsilon}{\lambda} =2L\beta B \| x^{k+1} - x^k\| \\
\implies  &\dist(0, \partial_x F(\hat x^{k+1}, w^{k+1})) \leq 2L\beta B \| x^{k+1} - x^k\|  + \left( L\beta B+ \frac{1}{\gamma} \right)\| \hat x^{k+1} - x^k\| \leq\left(3L\beta B  + \frac{1}{\gamma}\right)\| x^{k+1} - x^k\|.
\end{align*}

As for stationarity in the $w$, we have
\begin{align*}
 \partial_w F(\hat x^{k+1}, w^{k+1})&= (h_{i}(c_{i}(\hat x^{k+1})))_{i} - \partial (-g)^\ast(-w) \\
 &= 
(h_{i}(c_{i}( x^{k})))_{i} - \partial (-g)^\ast(-w)  + (h_{i}(c_{i}(\hat x^{k+1})) - h_{i}(c_{i}( x^{k})))_{i}
\end{align*}
which, upon observing that $ 0 \in (h_{i}(c_{i}( x^{k})))_{i} - \partial (-g)^\ast(-w)$, implies the distance bound.$\hfill\square$
\end{proof}










==> section_inexact.tex <==
\section{Inexact analysis}
\begin{algorithm}[H]
	\caption{ICPLAM: Inexact Composite Prox-linear Alternating Minimization
		\label{alg:COMP-PAM3}}
	\begin{algorithmic}[1]
		\Require{$x_0 \in \RR^{d},  \gamma>0 $.}
		% \Statex
		
		\Statex{Set $w^0=c(x^0)$.}
		
		\Statex{Generate triples $\{(x_{k},w_k,\varepsilon_k)\}$ satisfying the following.}
   \Statex{{\bf Step $k$:} $(k\geq 0)$}
		\Statex{ \label{alg:main:line_PG}$\qquad$ $w^{k+1} \in \am_{w} \; F(x^{k},w)$.}
		\Statex\label{alg:main:line_PL} 
		$\qquad$ $x^{k+1}$ is an $\varepsilon_{k+1}$-minimizer of the function $x\mapsto
		 F_{x^k}(x,w^{k+1})+\frac{1}{2\gamma_k} \|x - x^k\|^2$.
	\end{algorithmic}
\end{algorithm}


\begin{theorem}
	
\end{theorem}
\begin{proof}
	Let $\bar x^{k+1}$ be the true minimizer of $F_{x^k}(\cdot,w^{k+1})+\frac{1}{2\gamma_k} \|\cdot - x^k\|^2$. Then we deduce
	\begin{align*}
	F_{x^k}(x^{k+1},w^{k+1})+\frac{1}{2\gamma_k} \|x_{k+1} - x^k\|^2&\leq \varepsilon_{k+1}+F_{x^k}(\bar x^{k+1},w^{k+1})+\frac{1}{2\gamma_k} \|\bar x^{k+1} - x^k\|^2\\
	&\leq\varepsilon_{k+1}+F(\bar{x}^k,w^k)-\frac{1}{2\gamma_k}\|\bar x^{k+1}-x^k\|^2
	\end{align*}
\end{proof}
	


\subsection{Extrabullshit}

Consider the model
$$
\
$$

\subsection{When $c_i$ are linear.}
%\subsubsection{Parallel Partial Minimization}
Suppose that $c_i(x)=A_ix$ for each $i$. Fix an $(\alpha,\nu)$-penalty and define the function
$$F_{\nu}(x,w):=g(x)+\frac{\bar{L}}{m}\sum_{i=1}\frac{1}{\nu}\|A_ix-w_i\|^2+\frac{1}{m}\sum_{i=1}^m h_{i}(w_i).$$

Notice that for $\nu_+ > \nu$, we have
\begin{align*}
F_{\nu_+}(x, w) \leq F_{\nu} + \frac{\bar{L}}{m}\sum_{i=1}\left(\frac{1}{\nu_+} - \frac{1}{\nu}\right)\|A_ix-w_i\|^2
\end{align*}

Consider the following method.


\begin{algorithm}[H]
  \caption{CPAM: Composite Proximal Alternating Minimization
    \label{alg:COMP-PAM}}
  \begin{algorithmic}[1]
    \Require{$x_0 \in \RR^{d},  \gamma>0, C> 0$.}
   % \Statex
  
   \Statex{Set $w^0=Ax^0$.}
    \Statex{{\bf Step $k$:} $(k\geq 0)$}
        \Statex \label{alg:main:line_PG} $\qquad$ Choose $w^{k+1} \in \am_{w} \; F_{\nu_k}(x^{k},w)$
        \Statex $ \qquad $ Choose $\nu_{k+1} = \frac{1}{(k+2)^{1/3}}.$
 \Statex\label{alg:main:line_PL} $\qquad$ Set $x^{k+1} = \am_{x} \; F_{\nu_{k+1}}(x,w^{k+1})+ \frac{1}{2\gamma_k} \|x - x^k\|^2$
  \end{algorithmic}
\end{algorithm}

{\color{red} Below we're using $\nu_k = 1/(k+2)$. the best stepsize is $\nu_k = 1/(k+2)^{1/3}$.}


\begin{theorem}\label{thm:main_thm}
Let $B = \sum_{i=0}^\infty \tau_i$.
Then the iterates $(x_k,w_k)$ generated by Algorithm~\ref{alg:COMP-PAM} satisfy
\begin{equation}\label{eqn:summ}
\sum_{k=0}^{\infty} \frac{1}{\gamma_k}\|x^{k+1}-x^k\|^2\leq F(x^0)-F^* + \frac{\pi^2C \bar L}{6},
\end{equation}
where we set $\displaystyle F^*:=\lf_{k\to\infty} F(x^k,w^k)$. Moreover, the following approximate stationarity condition holds:
\begin{equation}\label{eqn:approx_stat}
\left\{\begin{aligned}
\dist\left(0, \partial g(x^{k+1})+ A^T\partial h(w^{k+1})\right) &\leq  \left(\frac{\bar{L}\sum_{i=1}^m\|A_i\|^2}{m \nu_k}+\frac{1}{\gamma_k}\right) \cdot\| x^k - x^{k+1} \| \\
 \|Ax^{k} - w^{k+1}\|_{\infty}&\leq \nu_k
\end{aligned}\right\}.
\end{equation}
\end{theorem}
\begin{proof}
 Using strong convexity of the function $F_{\nu_{k}}(\cdot,w^{k+1})+\frac{1}{2\gamma}\|\cdot-x^k\|^2$, for any index $k$, we deduce
\begin{align*}
&\left(F_{\nu_{k+1}}(x^{k+1},w^{k+1})+\frac{1}{2\gamma_k}\|x^{k+1}-x^k\|^2\right)+\frac{1}{2\gamma_k}\|x^{k+1}-x^k\|^2\\
&\hspace{20pt}\leq F_{\nu_{k+1}}(x^{k},w^{k+1})\\
&\hspace{20pt} \leq F_{\nu_k}(x^k, w^{k+1}) + \frac{\bar{L}}{m}\sum_{i=1}\left(\frac{1}{\nu_{k+1}} - \frac{1}{\nu_k}\right)\|A_ix^{k}-w^{k+1}_i\|^2\\
&\hspace{20pt}\leq F_{\nu_k}(x^{k},w^{k}) + \nu_k^2\bar{L}\left(\frac{1}{\nu_{k+1}} - \frac{1}{\nu_k}\right)\\
&\hspace{20pt}\leq F_{\nu_k}(x^{k},w^{k}) + \frac{C\bar L}{(k+1)^2} 
\end{align*}
Therefore, 
%$$
%F_{\nu_{k+1}}(x^{k+1}, w^{k+1}) \leq  F_{\nu_k}(x^k, w^k) - \frac{1}{\gamma_k} \|x^{k+1} - x^k\|^2 + \frac{\bar{L}}{m}\sum_{i=1}\left(\frac{1}{\nu_{k+1}} - \frac{1}{\nu_k}\right)\|A_ix^{k+1}-w^{k+1}_i\|^2.
%$$
Rearranging yields
$$\sum_{k=0}^N \frac{1}{\gamma}\|x^{k+1}-x^k\|^2\leq \sum_{k=0}^N \left(F(x^{k},w^{k})-F(x^{k+1},w^{k+1}) + \frac{C\bar L}{(k+1)^2}\right) \leq F(x^0,w^0)-F^* +\frac{\pi^2C \bar L}{6} .$$
Taking into account the equality $F(x_0)=F(x_0,w_0)$, we arrive at \eqref{eqn:summ}.

From the definition of $w^{k+1}$, we obtain the inclusions
\begin{equation}\label{eqn:exact_pen}
\bar{L}\nabla p_i(A_ix^{k} - w^{k+1}_{i}) \in \partial h_i(w^{k+1}_{i}),
\end{equation}
for each index $i$.
Since $p$ is a $(\alpha,\nu)$-penalty,  the inequality 
\begin{equation}\label{eqn:inf_est}
\|A_ix^{k} - w^{k+1}_i\|\leq \nu_k
\end{equation}
must hold for each index $i$. Multiplying \eqref{eqn:exact_pen} by $A_i^T$ and summing yields
\begin{equation}\label{eqn:summed_eqn}
\frac{\bar{L}}{m}\sum_{i=1}^m A_i^T\nabla p_i(A_ix^{k} - w^{k+1}_{i}) \in \frac{1}{m}\sum_{i=i}^m A_i^T\partial h_i(w^{k+1}_{i}).
\end{equation}
The definition of $x^{k+1}$, in turn, implies
\begin{equation}\label{eqn:main_inc_proof}
0\in \frac{\bar{L}}{m}\sum_{i=1}^m A_i^T \nabla p_i(A_ix^{k+1} - w^{k+1}_{i})  +\frac{1}{\gamma_k}( x^{k+1}-x^k)+\partial g(x^{k+1}).
\end{equation}
Taking into account that $p_i$ is $\frac{1}{\nu}$-Lipschitz yields 
\begin{equation}\label{eqn:lip_est}
\left\|\frac{1}{m}\sum_{i=1}^m A_i^T \nabla p_i(A_ix^{k+1} - w^{k+1}_{i})-\frac{1}{m}\sum_{i=1}^m A_i^T \nabla p_i(A_ix^k - w^{k+1}_{i})  \right\|\leq   \frac{\sum_{i=1}^m\|A_i\|^2}{m \nu} \cdot\| x^k - x^{k+1} \|.
\end{equation}
Combining the expressions \eqref{eqn:main_inc_proof} and \eqref{eqn:lip_est}, we conclude
\begin{equation}\label{eqn:dist_est}
\dist\left(0;\partial g(x^{k+1})+\frac{\bar{L}}{m}\sum_{i=1}^m A_i^T \nabla p_i(A_ix^k - w^{k+1}_{i})\right)\leq  \left(\frac{\bar{L}\sum_{i=1}^m \|A_i\|^2}{m \nu}+\frac{1}{\gamma_k}\right) \cdot\| x^k - x^{k+1} \|.
\end{equation}
Taken together, expressions \eqref{eqn:inf_est} and \eqref{eqn:dist_est} yield the  perturbed stationarity \eqref{eqn:approx_stat}, thereby completing the proof.$\hfill\square$
%\begin{align*}
%\frac{1}{\gamma}(x^k - x^{k+1}) = \frac{1}{m}\sum_{i=1}^m A_i^T \nabla p_i(A_ix^{k+1} - w^{k+1}_{i})  \in   \frac{1}{m}\sum_{i=1}^m A_i^T \nabla p_i(A_ix^k - w^{k+1}_{i})  + \frac{ \frac{1}{m}\sum_{i=1}^m\|A_i\|^2}{\nu} \| x^k - x^{k+1} \|B .
%\end{align*}
%Furthermore, because $h_i$ is $L$-Lipschitz, we have
%\begin{align*}
%\bar L \nabla p_i(A_ix - w_{i,+}) \in \partial h_i(w_{i,+}) \implies \|A_ix - w_{i,+}\| %\leq \alpha
%\end{align*}
%Clearly, this last upper bound also implies the subdifferential distance bound as well. 
\end{proof}


Combining \eqref{eqn:summ} and \eqref{eqn:approx_stat}, it is now straightforward to choose $\gamma$ optimally. 

\begin{corollary}\label{cor:main_comp}
For some $\bar L>L$ and define the quantity
$$Q_N:=\frac{(N+1)\bar{L}\sum_{i=1}^m\|A_i\|^2}{mC}$$
Then Algorithm~\ref{alg:COMP-PAM} with $\gamma_k:=\frac{1}{\sqrt{1+Q_k^2}}$ produces iterates $(x_k,w_k)$ satisfying
\begin{equation}\label{eqn:summability_res}
\left\{\begin{aligned}
\sum_{k=0}^{\infty}\|x^{k+1}-x^k\|^2+\dist^2\left(0, \partial g(x^{k+1})+ A^T\partial h(w^{k+1})\right) &\leq  2\left(Q_k+\sqrt{1+Q_k^2}\right)(F(x^0)-F^*) \\
 \|Ax^{k} - w^{k+1}\|_{\infty}&\leq \nu_k
\end{aligned}\right\},
\end{equation}
where we set $\displaystyle F^*:=\lf_{k\to\infty} F(x^k,w^k)$. Consequently, the method will find points $(x^{k},x^{k+1},w^{k+1})$ satisfying
\begin{equation}
\left\{\begin{aligned}
&\dist\left(0, \partial g( x^{k+1})+ A^T\partial h(w^{k+1})\right) \leq  \varepsilon \\
 &\|x^{k+1}- x^k\|\leq \varepsilon,\quad \|Ax^k - w^{k+1}\|_{\infty}\leq \alpha
\end{aligned}\right\},
\end{equation}
after at most 
\begin{equation}\label{eqn:complexity_fin}
N=\ceil*{\frac{2\left(Q_N+\sqrt{1+Q_N^2}\right)}{\varepsilon^2}(F(x^0)-F^* + \frac{\pi^2C \bar L}{6})}
\end{equation}
iterations.

\end{corollary}
\begin{proof}
Inequality \eqref{eqn:summ} combined with the first inequality in \eqref{eqn:approx_stat} directly imply 
\begin{align*}
\sum_{k=0}^{N}\|x^{k+1}-x^k\|^2+\dist^2\left(0, \partial g(x^{k+1})+ A^T\partial h(w^{k+1})\right)&\leq \left(\left(\frac{\bar{L}\sum_{i=1}^m\|A_i\|^2}{m \nu_{N+1}}+\frac{1}{\gamma_k}\right)^2+1\right)\gamma \cdot\sum_{k=0}^{N} \frac{1}{\gamma_k}\| x^k - x^{k+1} \|^2\\
&\leq \left(\left(\frac{\bar{L}\sum_{i=1}^m\|A_i\|^2}{m \nu_{N+1}}+\frac{1}{\gamma_k}\right)^2+1\right)\gamma_k \cdot (F(x^0)-F^* + B).
%&\leq \left(\frac{\bar{L}\sum_{i=1}^m\|A_i\|^2}{m \nu}+\frac{1}{\gamma}\right)^2(2\gamma) \cdot (F(x_0)-F^*).
\end{align*}
%Adding \eqref{eqn:summ} yields
%\begin{align*}
%\sum_{k=0}^{\infty}\|x^{k+1}-x^k\|^2+\dist^2\left(0, \partial g(x^{k+1})+ A^T\partial h(w^{k+1})\right)&\leq \left(\frac{\bar{L}\sum_{i=1}^m\|A_i\|^2}{m \nu}+\frac{1}{\gamma}\right)^2(2\gamma) \cdot\sum_{k=0}^{\infty} \frac{1}{2\gamma}\| x^k - x^{k+1} \|^2
%&\leq \left(\frac{\bar{L}\sum_{i=1}^m\|A_i\|^2}{m \nu}+\frac{1}{\gamma}\right)^2(2\gamma) \cdot (F(x_0)-F^*).
%\end{align*}
Minimizing the right-hand-side in $\gamma$ yields the choice 
$\gamma:=\frac{1}{\sqrt{Q_k^2+1}}$. With this choice of $\gamma$, the right-hand-side becomes $4\left(Q_k+\sqrt{1+Q_k^2}\right)$.
%$\gamma=\frac{m\nu}{\bar{L}\sum_{i=1}^m\|A_i\|^2}$.
%$\frac{8\bar{L}\sum_{i=1}^m\|A_i\|^2}{m \nu}(F(x_0)-F^*)$. 
The claimed guarantee \eqref{eqn:summability_res} follows. 


To simplify notation, henceforth set $r_{k+1}:=\dist\left(0, \partial g(x^{k+1})+ A^T\partial h(w^{k+1})\right)$. From \eqref{eqn:summability_res}, we deduce
$$\sum_{k=0}^{N} (\|x^{k+1}-x^k\|^2+r_{k+1}^2)\leq 2\left(Q_N+\sqrt{1+Q_N^2}\right)(F(x^0)-F^* + \frac{\pi^2C \bar L}{6}).$$
 We deduce 
\begin{align*}
\min_{k=0,1,\ldots,N-1}~ (\|x^{k+1}-x^k\|^2+r_{k+1}^2)&\leq \frac{1}{N}\sum_{k=0}^{N-1} (\|x^{k+1}-x^k\|^2+r_{k+1}^2)\\
&\leq \frac{2\left(Q_N+\sqrt{1+Q_N^2}\right)}{N}(F(x^0)-F^* + \frac{\pi^2C \bar L}{6}).
\end{align*}
 Setting the right-hand-side equal to $\varepsilon^2$ and solving for $N$ yields the claimed complexity \eqref{eqn:complexity_fin}.

$\hfill\square$
\end{proof}


Random bullshit.
Let $$h(w)=\frac{1}{m}\sum_{i=1}^m |b_i-|w_i||=\frac{1}{m}\sum_{i=1}^m \min\{|w_i-b_i|,|w_i+b_i|\}.$$
Suppose $x^*$ is a solution to the phase retrieval problem (whp $\pm x^*$ are the only solutions) and set $w^*=Ax^*$. Suppose $|\Delta_i|\leq |b_i|$ and set $w=w^*+\Delta$. Then $$\min\{|w_i-b_i|,|w_i+b_i|\}=\min\{|w_i-w_i^*|,|w_i+w_i^*|\}$$ Therefore 
$h(w)\geq \frac{1}{m}\dist_{\ell_1}(w;{\pm w^*})$.


\begin{lemma}[Error bound for Sign Retrieval Loss]
Let $h(w) = \||w^\ast| - |w|\|_1$. Suppose that $|w_i - w_i^\ast|  \leq (3/2) |w^\ast_i|$. Then 
\begin{align*}
h(w) \geq \frac{1}{3}\|w - w^\ast\|_1
\end{align*}
In other words the above bound holds in the $\|\cdot\|_{w^\ast, \infty}$-ball of radius $3/2$. 

Moreover, suppose that $|w_i^\ast| = 1$ for all $i$. Then the condition $|w_i - w_i^\ast|  \leq (3/2) |w^\ast_i|$ is implied by 
$$
\|w - w^\ast\| \leq \frac{3}{2}.
$$
\end{lemma}
\begin{proof}
Case 1:  $\sign(w_i) = \sign(w_i^\ast)$. Then
\begin{align*}
||w_i^\ast| - |w_i|| = |w_i^\ast - w_i|.
\end{align*}
Case 2: $w_i^\ast > 0$ and $w_i \in [-(1/2)w_i^\ast, 0]$. Then 
\begin{align*}
||w_i^\ast| - |w_i|| \geq \frac{1}{2}|w_i^\ast| \geq \left(\frac{1}{2}\cdot \frac{2}{3}\right) \frac{3}{2}|w_i^\ast| \geq \frac{1}{3}|w_i^\ast - w_i|
\end{align*}
Case 3: $w_i^\ast < 0$ and $w_i \in [0, -(1/2)w_i^\ast]$. Same proof to Case 2.
\end{proof}

\begin{proposition}
Define a function $ f(w) = \frac{\ell}{2} d_{\mathrm{Im}(A)}^2(w)$ and $F(w) := f(w) + h(w)$. Then  ??
\end{proposition}
\begin{proof}
Let $t+1$ be the first iterate such that for some $i$, we have
\begin{align*}
|y_i^{k+1} - y_i^\ast| > \frac{3}{2}|y_i^\ast|.
\end{align*}
\begin{lemma}
Suppose that we have for all $ t \leq k-1$, the bound
\begin{align*}
\|y^t - y^\ast\|_1 < \frac{2}{3\ell} \qquad  \text{ and } \qquad \left(\forall t\right) \;  |y_i^\ast - y^{t}_i| \leq \frac{3}{2}|y_i^\ast| \qquad  \text{ and } F(y^t) - F(y^\ast) < \frac{18}{\ell}
\end{align*}
For all $t \leq k-1$, the following holds
   \begin{align*}
   \left(t \leq k\right) & \qquad   \|y^{t} - y^\ast\|_1 \leq \left(\frac{3\ell}{2}\right)^{-1} \left(\frac{3\ell}{2} \|y^0 - y^\ast\|_1\right)^{2^{t}} \\
 \left(t \leq k+1\right) & \qquad F(y^{t}) - F(y^\ast) \leq \left(\frac{\ell}{18}\right)^{-1} \left(\frac{\ell}{18} \left[F(y^0) - F(y^\ast)\right]\right)^{2^{t}}
  \end{align*}
  \end{lemma} 
  
  \begin{lemma}
  For all $t$, we have 
\begin{align*}
  F(y^{t+1}) &\leq F(y^t) - \frac{\ell - \beta}{2}\|y^{t+1}-y^t\|^2  \\
  \|y^{t+1}-y^\ast\| &\leq \sqrt{\frac{2}{\ell - \beta}(F(y^t) - F(y^{t+1}))} + \|y^t - y^\ast\|  .
\end{align*}
  \end{lemma}
  
  
  Plugging all this shit together, we find that 
   \begin{align*}
   |y_i^{k+1} - y_i^\ast|  \leq \|y^{k+1}-y^\ast\| &\leq \sqrt{\frac{2}{\ell - \beta}(F(y^k) - F(y^{k+1}))} + \|y^k - y^\ast\| \\
   &\leq \sqrt{\frac{2}{\ell - \beta} \left(\frac{\ell}{18}\right)^{-1} \left(\frac{\ell}{18} \left[F(y^0) - F(y^\ast)\right]\right)^{2^{k}}} + \left(\frac{3\ell}{2}\right)^{-1} \left(\frac{3\ell}{2} \|y^0 - y^\ast\|_1\right)^{2^{k}}\\
   &\leq \frac{3}{2}|y_i^\ast|.
   \end{align*}
   So at $k= 0$, we need 
   \begin{align*}
   &\frac{3}{2}|y_i^\ast| \\
   &\geq \sqrt{\frac{2}{\ell - \beta} \left(\frac{\ell}{18}\right)^{-1} \left(\frac{\ell}{18} \left[F(y^0) - F(y^\ast)\right]\right)} + \left(\frac{3\ell}{2}\right)^{-1} \left(\frac{3\ell}{2} \|y^0 - y^\ast\|_1\right)\\
      &= \sqrt{\frac{2}{\ell - \beta}  \left[F(y^0) - F(y^\ast)\right]} +  \|y^0 - y^\ast\|_1
   \end{align*}
  
  
  
    \begin{proof}[of Lemma]
Method ($\nabla f$ is $\beta$ lipschitz, $\ell \geq \beta$).
$$y^{t+1}\in\am_{y}~ \{f(y^t)+\dotp{\nabla f(y^t),y-y^t}+h(y)+\tfrac{\ell}{2}\|y-y^t\|^2\}.$$


Then two bound
\begin{align*}
F(y^{t+1})&\leq f(y^t)+\dotp{\nabla f(y^t),y^{t+1}-y^t}+h(y^{t+1})+\tfrac{\ell}{2}\|y^{t+1}-y^t\|^2\\
&\leq  f(y^k)+\dotp{\nabla f(y^t),y^{*}-y^t}+h(y^{*})+\tfrac{\ell}{2}\|y^{*}-y^t\|^2\\
&\leq F(y^\ast) +\tfrac{\ell}{2}\|y^{*}-y^t\|^2\\
&\leq F(y^\ast) + \frac{\ell}{18} \left[F(y^t) - F(y^\ast)\right]^2 %- \frac{1}{9}f(y^t) h(y^t) - \frac{1}{18}f(y^t)^2,
\end{align*}
and the second bound
\begin{align*}
F(y^{t+1})&\leq F(y^\ast) +\tfrac{\ell}{2}\|y^{*}-y^t\|^2\\
&\leq F(y^\ast) +\ell\|y^{*}-y^t\|^2 - \tfrac{\ell}{2}\|y^{*}-y^t\|^2\\
&\leq F(y^\ast) + \frac{\ell}{9} \left[F(y^t) - F(y^\ast)\right]^2 - \tfrac{\ell}{2}\|y^{*}-y^t\|^2
\end{align*}
where we use the bound 
$$
\|y^{*}-y^t\|^2 \leq \|y^{*}-y^t\|_1^2 \leq \frac{1}{9}h^2(y^t) \leq   \frac{1}{9}(h(y^t) + f(y^t))^2% - \frac{2}{9}f(y^t) h(y^t) - \frac{1}{9}f(y^t)^2.
$$
Therefore, 
\begin{align*}
(F(y^{t+1}) - F(y^\ast)) \leq \frac{\ell}{18} \left[F(y^t) - F(y^\ast)\right]^2 % \frac{1}{9}f(y^t) h(y^t) + \frac{1}{18}f(y^t)^2 
\end{align*}
So we get quadratic convergence as long as 
$$
\frac{\ell}{18} \left[F(y^t) - F(y^\ast)\right] < 1 \implies F(y^t) - F(y^\ast) < \frac{18}{\ell}.
$$
Likewise we have
\begin{align*}
  \tfrac{\ell}{2}\|y^{*}-y^t\|^2 \leq \frac{\ell}{9} \left[F(y^t) - F(y^\ast)\right]^2 - (F(y^{t+1}) - F(y^\ast))
\end{align*}
We need the bound 
$$
|y_i^{t+1} - y_i^\ast| \leq \frac{3}{2}|y_i^\ast|
$$
 to continue getting it.
 We have that, 
 \begin{align*}
 \|y^{t+1} - y^\ast\|_1\leq \frac{3\ell}{2}d^2_{\mathrm{Im}(A)}(y^{t+1}) + 3h(y^{t+1}) \leq 3(F(y^{t+1}) - F(y^\ast) )\leq \frac{3\ell}{2}\|y^t - y^\ast\|_2^2  \leq \frac{3\ell}{2}\|y^k - y^\ast\|_1^2.
 \end{align*}
 Length of $ y^t$ path:
 \begin{align*}
 \|y^{t+1} - y^\ast\|_1 \leq \left(\frac{3\ell}{2}\right)^{-1} \left(\frac{3\ell}{2} \|y^0 - y^\ast\|_1\right)^{2^{t+1}} 
  \end{align*}
  We need 
  \begin{align*}
  |y_i^{t+1} - y_i^\ast| \leq  \left(\frac{3\ell}{2}\right)^{-1} \left(\frac{3\ell}{2} \|y^0 - y^\ast\|_1\right)^{2^{t+1}}  &\leq \frac{3}{2}|y_i^\ast|
  \end{align*}
  Thus, we just need to show that
  \begin{align*}
   &\left(\frac{3\ell}{2} \|y^0 - y^\ast\|_1\right)^{2}  \leq \ell \left(\frac{3}{2}\right)^2|y_i^\ast|\\
   &\implies \frac{3\ell}{2} \|y^0 - y^\ast\|_1 \leq \sqrt{\ell} \left(\frac{3}{2}\right)\sqrt{|y_i^\ast|}\\
      &\implies \|y^0 - y^\ast\|_1 \leq \frac{1}{\sqrt{\ell}}\sqrt{|y_i^\ast|}.
  \end{align*}
 \end{proof} 
 
 \begin{proof}[of second lemma]
  Then one bound
\begin{align*}
F(y^{k+1})&\leq f(y^k)+\dotp{\nabla f(y^k),y^{k+1}-y^k}+h(y^{k+1})+\tfrac{\ell}{2}\|y^{k+1}-y^k\|^2 - \frac{\ell - \beta}{2}\|y^{k+1}-y^k\|^2\\
&\leq F(y^k) - \frac{\ell - \beta}{2}\|y^{k+1}-y^k\|^2 \\
\implies &  \frac{\ell - \beta}{2}\|y^{k+1}-y^k\|^2 \leq F(y^k) - F(y^{k+1})\\
\implies &  \|y^{k+1}-y^k\| \leq \sqrt{\frac{2}{\ell - \beta}(F(y^k) - F(y^{k+1}))}\\
\implies &  \|y^{k+1}-y^\ast\| \leq \sqrt{\frac{2}{\ell - \beta}(F(y^k) - F(y^{k+1}))} + \|y^k - y^\ast\|  
\end{align*}  
 \end{proof}
\end{proof}
%\begin{lemma}
%\textcolor{red}{Fill in later}
%
%Suppose that $(x^\ast, w^\ast)$ is $\frac{\varepsilon}{m}$-stationary for Problem~\eqref{eqn:exact_pen}, with $\varepsilon< \overline{L}-L$. Then the there exists $y$ satisfying
%$$\dist_{\infty}(y,\partial h(c(x)))\leq \frac{\varepsilon}{m}\qquad \textrm{ and }\quad \dist_2(0;\nabla c(x)^*y+\partial g(x))\leq \frac{\varepsilon}{m}.$$
%
%%$$0 \in \partial g(x^\ast) + \nabla c(x^\ast)^T\partial h(c(x^\ast))\qquad \textrm{holds}.$$
%
%
%\end{lemma}
%\begin{proof}
%$$
%\partial F(x,w)= \overline{L} \begin{bmatrix} \nabla c(x)^* \\ -I \end{bmatrix}\partial \|\cdot\|_1(c(x)-w)+\begin{bmatrix} \partial g(x)\\
%\partial h(w)\end{bmatrix}.
%$$
%There exists a vector $v\in \partial \|\cdot\|_1(c(x)-w)$ satisfying 
%$$\dist_2(0;\nabla c(x)^*(\overline{L}v)+\partial g(x))\leq \frac{\varepsilon}{m}\quad \textrm{and}\quad \dist_{\infty}(0;-\overline{L}v+\partial h(w))\leq \frac{\varepsilon}{m}$$
%
%Hence $\dist(0;\frac{\bar{L}}{m}\partial \|\cdot\|(c_i(x)-w_i)+\frac{1}{m}\partial h_i(w_i))\leq \frac{\varepsilon}{m}$. If $c_i(x)\neq w_i$, then $\partial \|\cdot\|(c_i(x)-w_i)$ is a unit vector, and therefore $\dist(0;\frac{\bar{L}}{m}\partial \|\cdot\|(c_i(x)-w_i)+\frac{1}{m}\partial h_i(w_i))\geq \frac{\overline{L}-L}{m}$. We deduce $\varepsilon\geq \overline{L}-L$, a contradiction. Thus $w_i=c_i(x)$ for all $i$.
%\end{proof}


